Defending From Physically-Realizable Adversarial Attacks Through Internal Over-Activation Analysis

This work presents Z-Mask, a robust and effective strategy to improve the adversarial robustness of convolutional networks against physically-realizable adversarial attacks. The presented defense relies on specific Z-score analysis performed on the internal network features to detect and mask the pixels corresponding to adversarial objects in the input image. To this end, spatially contiguous activations are examined in shallow and deep layers to suggest potential adversarial regions. Such proposals are then aggregated through a multi-thresholding mechanism. The effectiveness of Z-Mask is evaluated with an extensive set of experiments carried out on models for both semantic segmentation and object detection. The evaluation is performed with both digital patches added to the input images and printed patches positioned in the real world. The obtained results confirm that Z-Mask outperforms the state-of-the-art methods in terms of both detection accuracy and overall performance of the networks under attack. Additional experiments showed that Z-Mask is also robust against possible defense-aware attacks.

==> checklist.tex <==
\onecolumn
\begin{center}
    \Huge\bf
    Checklist
\end{center}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The paper presents the \NAME~tool and an extensive set of experiment on a set of dataset generated with \NAME. Both contributions are presented in the main paper (Section \ref{s:proposed}-\ref{s:exp}) and better detailed in the supplementary material (Section 2).}
  \item Did you describe the limitations of your work?
    \answerYes{Section \ref{s:conclusions} reports an analysis of a few limitations of the approach.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Section \ref{s:intro} briefly goes through the security and safety concerns.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\end{enumerate}


This paper:

    clearly states what claims are being investigated (yes/partial/no)
    explains how the results substantiate the claims (yes/partial/no)
    explicitly identifies limitations or technical assumptions  (yes/partial/no)
    includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)

Does this paper make theoretical contributions? (yes/no)

If yes, please complete the list below.

    All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
    All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    Proofs of all novel claims are included. (yes/partial/no)
    Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    Appropriate citations to theoretical tools used are given. (yes/partial/no)

Does this paper rely on one or more data sets? (yes/no)

If yes, please complete the list below.

    All novel datasets introduced in this paper are included in a data appendix (yes/partial/no/NA)
    All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes (yes/partial/no/NA)
    All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations (yes/no/NA)
    All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available (yes/partial/no/NA)
    All datasets that are not publicly available are described in detail (yes/partial/no/NA)

Does this paper include computational experiments? (yes/no)

If yes, please complete the list below.

    All source code required for conducting experiments is included in a code appendix (yes/partial/no).
    All source code required for conducting experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes (yes/partial/no)
    If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
    This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
    This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics (yes/partial/no)
    This paper states the number of algorithm runs used to compute each reported result (yes/no)
    Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information (yes/no)
    This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments (yes/partial/no/NA)
    This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)

